InfiniCache: Exploiting Ephemeral Serverless Functions to Build a Cost-Effective Memory Cache

Internet-scale web applications are becoming increasingly storage-intensive and rely heavily on in-memory object caching to attain required I/O performance. We argue that the emerging serverless computing paradigm provides a well-suited, cost-effective platform for object caching. We present InfiniCache, a first-of-its-kind in-memory object caching system that is completely built and deployed atop ephemeral serverless functions. InfiniCache exploits and orchestrates serverless functions' memory resources to enable elastic pay-per-use caching. InfiniCache's design combines erasure coding, intelligent billed duration control, and an efficient data backup mechanism to maximize data availability and cost-effectiveness while balancing the risk of losing cached state and performance. We implement InfiniCache on AWS Lambda and show that it: (1) achieves 31 -- 96X tenant-side cost savings compared to AWS ElastiCache for a large-object-only production workload, (2) can effectively provide 95.4% data availability for each one hour window, and (3) enables comparative performance seen in a typical in-memory cache.

==> Makefile <==
.SUFFIXES: .tex .dvi .ps .fig .eps .gnu .c
#PDF = ps2pdf -dPDFSETTINGS=/printer -dMaxSubsetPct=100 -dCompatibilityLevel=1.4 -dSubsetFonts=true -dEmbedAllFonts=true -sPAPERSIZE=letter -dUseCIEColor
PDF = ps2pdf14 -dPDFSETTINGS=/prepress -dEmbedAllFonts=true \
	       -dSubsetFonts=true -dMaxSubsetPct=100

TARGET=paper
DOBIB=yes
VIEWER=evince

HOST=$(shell hostname)

.PHONY: $(TARGET)

all:	display


display: $(TARGET)
	#dvips -Ppdf -G0 $(TARGET).dvi -o $(TARGET).ps
	pdflatex $(TARGET).tex
	#$(PDF) $(TARGET).ps
#ifeq ($(USER),  butta)
#	evince paper.pdf
#endif
#ifeq ($(HOST),  uet)
#	evince paper.pdf
#else
#	open paper.pdf
#endif

#display: $(TARGET)
#	dvips -Ppdf -G0 $(TARGET).dvi -o $(TARGET).ps
#	$(PDF) $(TARGET).ps
#	$(VIEWER) $(TARGET).pdf

$(TARGET): $(TARGET).tex
#	latex $(TARGET)
	pdflatex $(TARGET)
ifeq ($(DOBIB),yes)
	bibtex $(TARGET)
	pdflatex $(TARGET)
	pdflatex $(TARGET)
endif

clean:
	$(RM) $(TARGET).ps $(TARGET).pdf $(TARGET).log $(TARGET).out $(TARGET).aux $(TARGET).dvi $(TARGET).tex.flc
	$(RM) $(TARGET).bbl $(TARGET).blg
	$(RM) *.kill kill*

purge:	clean
	$(RM) *~

nums:
	cd numbers;gnuplot plotGraph

spell:
	cat $(TF) | awk '{ if (index($$0,"%")!=1) print $$0}' |  spell 
#	detex $(TF) |  spell 

strip: $(TARGET)
	mkdir -p stripped/source
	for a in `ls --color=auto *.tex`; do cat $$a | awk '{ if (index($$0,"%")!=1) print $$0}' >stripped/source/$$a; done
	(cd stripped/source; \
	cat paper.tex | awk '{if (match($$0, "\\input")==0) print $$0; else {sub( /}/, ".tex", $$xx); sub(/\\input{/, "", $$xx);  system("cat " $$xx);}}'  > step1; \
	rm *.tex; \
	mv step1 paper.tex; \
	cp ../../paper.bbl .; \
	cd ../..)
	pwd
	(cd stripped/source; files=`ls --color=auto *.eps`; \
	cd ../..; cp $$files stripped/source/; )
	(for dirs in figure plot2 plot3; \
	do cd stripped/source/$$dirs; \
	files=`ls --color=auto *.eps`; \
	cd ../../../$$dirs; \
	cp $$files ../stripped/source/$$dirs; \
	cd ..; \
	done )



==> impl.tex <==
\vspace{-6pt}
\section{Implementation}
\label{sec:impl}
\vspace{-5pt}


